On Image segmentation using Fractional Gradients-Learning Model Parameters using Approximate Marginal Inference

Estimates of image gradients play a ubiquitous role in image segmentation and classification problems since gradients directly relate to the boundaries or the edges of a scene. This paper proposes an unified approach to gradient estimation based on fractional calculus that is computationally cheap and readily applicable to any existing algorithm that relies on image gradients. We show experiments on edge detection and image segmentation on the Stanford Backgrounds Dataset where these improved local gradients outperforms state of the art, achieving a performance of 79.2% average accuracy.

==> CVPR /FOC.tex <==
\section{Fractional Order Calculus Overview}
\label{sec:FOC}

It is actually a more simplified framework rather a subset of the complex Calculus which says that Diff-integral operators can take any complex value. thus, the integer order diff-Integral operators belong to the integer domain which lies inside a single Riemann Sheet  of Fractional domain which in turn falls within the superset of complex calculus.\\
In spite of the fact that fractional order calculus was introduced 300 years ago but still most of the notions remain unclear and unrealizable. For example, if one considers a filter of orer 1 it implies 1 pole in the integer oreder Frequency domain, but it might be mapped as $\frac{10}{10}$ i.e. 10 poles distributed over 10 riemann sheets , both seem to give similar response thus are equivalent. Thus, on a higher level it can be said

\begin{equation}
\{Integer Domain\} \subseteq \{Fractional Domain\} \subseteq \{Complex Domain\}
\end{equation}


"Fractional Calculus is a field of applied mathematics that deals with
derivatives and integrals of arbitrary
orders (including complex orders), and
their applications in science, engineering, mathematics, economics, and
other fields" [4]
The idea of Fractional Calculus dates back to 17th Century. The term was first coined by L'Hospital to Leibnitz while discussing about the possible interpretation of his derivation of $n^{th}$ order derivative.[2] And the first breakthrough was provided by Liebnitz when he introduced a possible approach to Fractional Order Differentiation(1697) \\
\begin{equation}\frac{d^n e^{mx}}{dx^n}=m^ne^{mx} \end{equation}
\\
Later Euler(1730)  suggested using the relationship for negative or non integer(rational) values for m=1 and n=1/2;
\\
\begin{equation}\frac{d^n x^m}{dx^n}=\frac{\Gamma (m+1)}{\Gamma (m-n+1)}x^{m-n}\\ \frac{d^{1/2}x}{dx^{1/2}}=\frac{2x^{1/2}}{\sqrt{\pi}} \end{equation}\\
While Euler proved it for specific value n=1/2 it was still not sure whether it exist for all the fractional orders and if there is something that can be applied generally and the first step in generalizing the concept for any non-integer order was given by Fourier (1820-1822) when he proposed the general n th order differentiation is given as\\
\begin{equation}\frac{d^nf(x)}{dx^n}=\frac{1}{2\pi}\int_{-\infty}^{\infty}f(z)dz\int_{-\infty}^{\infty}p^ncos(px-pz+n\frac{\pi}{2})dp \end{equation} 
\\
Since then many top Mathematicians (Pure and Applied) of their times have contributed significantly in this field namely N. H. Abel, M. Caputo, L. Euler, J. Fourier, A. K. Grunwald J. Hadamard, G. H. Hardy, O. Heaviside, H. J. Holmgren,
P. S. Laplace, G. W. Leibniz, A. V. Letnikov, J. Liouville, B. Riemann
M. Riesz, and H. Weyl etc.[4]. 

\subsection{Popular Fractional Differ-Integrals}
The main results on fractional Diff-Integrals that are widely used and popular are provided briefly.[1][2]
\subsubsection{Grunwald–Letnikov (G–L) definition}
This is basically an extension of the backward finite
difference formula for successive differentiation. This
formula is used widely for the numerical solution of
fractional differentiation or integration of a function.
According to Grunwald–Letnikov definition the $\alpha^{th}$ order differ-integration of a function f(t) is defined as 
\begin{equation}
D_t^{\alpha}f(t)=lim_{h\rightarrow 0}\frac{1}{h^{\alpha}}\sum_{j=0}^{\infty}(-1)^j \frac{\Gamma(\alpha +1)}{\Gamma(j+1)\Gamma(\alpha-j+1)}f(t-jh)
\end{equation}
\subsubsection{ Riemann–Liouville (R–L) definition}
This is an extension of n-fold successive integration. The $\alpha$-th order differentiation of f(t) is defined as 
\begin{equation}
D_t^{\alpha}f(t)=\frac{1}{\Gamma(n-\alpha)}\frac{d^n}{dt^n}\int_{\alpha}^{t}\frac{f(\tau)}{(t-\tau)^{\alpha -n +1}}d\tau   
\end{equation}


==> CVPR /imsegment.tex <==
\section{Fractional Order Derivative of Gaussian Filters for Edge Detection}
\label{sec:imsegment}

\iffalse
In the computer vision community, most of the research in image segmentation is geared towards enhancing the performance of the segmentation task in order to match, or even better that of humans. A good contrast between the different segmentation algorithms can be found in~\cite{amfm_pami2011}. In general, any image segmentation can be conceived as a machine learning task with wise feature selection and image processing~\cite{937655,1273918,fowlkes2004much}, and can be summarized by the following steps:
\begin{itemize}
\item Pre-rocessing of the input image, e.g. denoising.
\item Finding good similarity cues that can be used to construct good affinity score metric. 
\item Clustering similar cues using some learning approach.
\end{itemize}
The overall performance of the segmentation process depends on the performance of each of the individual steps mentioned above, and their efficient inter operability. We analyze each of these steps and propose a simple and efficient approach to combine them in order to enhance segmentation performance. 
%analyses each of these steps and pr and tries to come up with a combination that would improve the overall segmentation result without giving up much on the Computational Complexity. So, the intuition is that if one can significantly improve each of these step without compromising much on the question of Computational complexity it is expected to improve the overall result on image segmentation. So, in the rest of the article we consider each step separately and try to find the optimal method with all the considerations and key constraints to be kept in mind in terms of Image Segmentation task and proceed to the next step and proceed like this till the end. 


\subsection{Finding Good Affinity Measures}
As mentioned above, identifying a set of good features plays an important role in segmentation. Most of the recent works rely on gradient based methods on color and texture maps, which is a reasonable approach in identifying important features as gradients often correspond to edges and hence likely segmentation boundaries in an image. Edge detection is a well researched problem and while there exists pretty reliable methods to do the same, these are more often than not computationally complex, slow in performance, and hence practically unusable for segmentation~\cite{Lafferty:2001:CRF:645530.655813,}.
%As discussed before the whole idea of any Segmentation Task is to come up with a set of good discriminative features which serves as feature space and  give strong discriminative power to the Clustering Algorithm. Often this is the most challenging and important part of image segmentation task. This is the most tricky part of any computer vision problem and should be given due importance. Past few years have noticed many research in the area of new classification or clustering algorithms ranging from improvenment of existing Learning algorithms as well as many Graph based and Spectral Clustering Algorithms. However, there has not been significant improvement in the feature extraction and selection algorithms. Most of the recent developemnet in this area has been done in late 90's [8] or early 20's [7][8]. Most of the more recent image segmentation algorithms use Gradient based approaches on Texture or color maps as done in [7]. \\
%However, most of the recent work shows succesfull segmentation results based on gradient based features. This is intuitively reasonable since edges in an image often reveals the location of the segmentation boundaries and thus thus it is very reasonable to consider gradient based approaches. Thus we first look to construct a better Edge Detector as the first step of the Segmenation task.
%\\ This paper adresses this issue of a good edge detection scheme which is often not given a very high importance while designing a segmentation algorithm. Though there are many nice edge detection[8] methods already designed but none of them are practical in the scenario of a image segmentation. The reason being that all of them increase the runtime complexity. The state-of-the-art segmentation algorithms being mostly based on Graph Structured models where inferencing itself is computationally difficult and often Exponential and thus most ofthe time is spent doing approximating the inferencing using approximate inferencing techniques such as Loopy Belief Propagation, MCMC or other approximate or sampling based algorithms[17][18][19][20][21]. These approximate algorithms often have high computational complexity. That being the case, the feature designing has to be computationally efficient to be of practical use. 
The most simple gradient computation scheme is based on calculating first order gradients with a Gaussian kernel based smoothing function [5],[6],[10],[11],[12],[16]. Though algorithms like anisotropic diffusion (ref) gives slightly better results, the payoff is not much considering the huge increase in computational complexity. We propose a new, efficient gradient computation method using concepts from fractional calculus which leverages the simplicity of kernel based gradient computations at a low computational complexity. The design of the filter kernels is described in the next section~\ref{subsec:filterkernels} and section ? evaluates the performance of application of this filter bank on practical images.
%leads to an gradient based approach that will improve the Gradient Feature quality and as a result the segmentation result without increasing the Computational Cost. The detailed descriptions of the algorithm with adequate justifications and comparison with other existing methods under similar settings is provided in the next section. We also propose a cheap and ready to use optimization technique to choose the optimal filter order under the assumption that the goal is a image segmentation, object detection, stereo matching or some other higher vision task being performed on a standard reasonably large dataset. The examples provided in this paper are evaluated on the Berkley Image Segmentation Dataset.   


\subsection{Improved Filter Bank for Gradient Calculation}
\label{subsec:filterkernels}
\fi
%In order to justify the design of the proposed Gradient Approximation algorithm a short review of the desirable objecties of an edge detection scheme is provided. This is crucial to understand underlying motivation and the strong justification on why the proposed method should always work and often lead to better solution.\\ 
%The basic goal of an edge detector is to reduce the amount of data in an image while preserving the structural properties as much as possible.[9].The basic motivation comes from the creation of a painting. Since, the first and foremost thing done by the artist while creating a painting is drawing the outline sketches or the boundaries. Thus, the edges which define the boundaries of an image gives us the most important structural information about an image which is often very descriptive feature of the image. That being the case, edge detection is the first step in most of the Computer Vision problems. \\

The most fundamental structural information embedded in an image is its edges. Edge detection is a well established notion in Computer Vision and is still a significant area of research. Among the various algorithms used for edge detection, detectors like Canny~\cite{Canny:1986:CAE:11274.11275}, Sobel, Pretwitt, Robert's Cross are particularly popular, Canny being the most reliable and widely used in the community.
Recently, the works of Perona, Malik et.al., based on  Anisotropic Diffusion algorithm~\cite{Perona:1990:SED:78302.78304}, and a new edge detection scheme proposed by Harris et.al.~\cite{Harris88alvey},  also gained popularity. However, one major disadvantage of Harris Detector is that it is not scale invariant. Though there has been many recent advances on the improvement of this~\cite{Brown:2005:MMU:1068507.1068957,Chum:2005:MPP:1068507.1068918}, most of these techniques are computationally complex compared to the Canny as well as Anisotropic Diffusion based detectors. These detectors might be extremely efficient when the sole task is edge detection. However, when we are concerned with a broader problem such as segmentation, edge detection is one of the many steps involved, and we need a robust and efficient detector without much overhead of computational complexity. %In other words, we need a detector which will maximize the signal to noise ratio (SNR) in terms of detected edges, should be locally scalable and have sparse peaks in a fixed neighborhood. 
%Thus in order to find a good edge detection scheme without much increase in computational complexity we  consider the following constraints/criterions to measure the edge detector performance.

\iffalse
\begin{itemize}
\item {\bf Good Detection} The detector should not miss any valid edges and should reveal as much structural information as possible, i.e. the filter should have high signal to noise ratio (SNR) given by, SNR= $\frac{\mid (f*S)(x_0)\mid}{\sigma_n\sqrt{\sum_kf^2(k)}}$, where $S$ is the input image minus the noise, $f$ is the impulse response of the filter and $\sigma_n$ is the variance of noise. The filter that maximizes the inner product is ideal for detection. 
\item {\bf Localization} A good detector should minimize the root mean squared error between a true edge location and the closest peak.
%The idea is to minimize the RMSE between the true edge location and the closest peak. Which is same as\\ minimizing $\sqrt{E(min_k\mid x_l^* -x_0\mid^2)}$ where $x_l^*$ is the local maxima in the response magnitude. 
%\\This is same as maximize SNR.LOC=$\frac{\mid (f*S)(x_0)\mid}{\sigma_n\sqrt{\sum_kf^2(k)}}\frac{1}{\sqrt{E(min_k\mid x_l^* -x_0\mid^2)}}$ The optimal filter will again be matched filter as befofre. 
\item {\bf Sparse Peaks} Now basically a good detection should not give too many peaks at the same neighbourhood and thus the added constraint to the above optimization problem is to find the optimal setting under this constraints\\
So, the optimization task is to \\
maximize SNR.LOC=$\frac{\mid (f*S)(x_0)\mid}{\sigma_n\sqrt{\sum_kf^2(k)}}\frac{1}{\sqrt{E(min_k\mid x_l^* -x_0\mid^2)}}$ \\s.t. $E[\mid_{k+1}^*-x_k^*]=x_{Peak}$ where $x_{Peak}$ is a design choice.\\
Sparsity of edge detector responses is a critical design criteria, It encourages a smooth envelope round the edges, and thereby less power at high frequencies. Which proves the necessaty of LPF before applying the gradient detectors. 
\end{itemize}
\fi

%The most commonly used Image Smoothing techniques in recent literatures is the Gaussian Kernel Based approach. This is a very reasonable approximation which makes a good trade off between all these three points mentioned. If instead one just solves for the max of the PSNR it would result in Box Shaped Kernel which suffers from non-satisfiability of Localization criterion. However, the detection should be scale invariant and a better approximation to that goal may be [8] as compared to scale space invariant smoothing introduced in [16].
An optimal edge detector captures the underlying geometric structure of the image (i.e. detects all the edges successfully) without being much affected by the noise present. As has been already shown by Canny et.al.~\cite{Canny:1986:CAE:11274.11275}, it is impossible to realize such an optimal filter for edge detection, although the first order gradient of Gaussians is a good approximation with around  20\% error. The order of the filter gradient is directly proportional to the number of detected edges and the amount of detected noise. Thus we get more peaked response at an edge with the second order LOG (Laplacian of Gaussian) as compared to the first order DOG (derivative of gaussian), with an additional side-effect of a higher response to noisy peaks for LOG as compared to DOG. In order to control this trade-off more efficiently, we propose a detector with fractional order gradient operator (FDOG) and show that the edge detection performance can be improved by using FDOG. 

%In general, the goal of an edge detector is to capture the underlying geometric structure of the image without being much affected by the noise present.  However, as it turns out to be these two are inversely related and one cannot do well on both. The response to edges increase as the order of the gradient operator increase, i.e.  
%However, while calculating the gradient features one is restrictes to the choice of DOG or LOG as other higher order derivatives would be too much susciptible to noise. \\ Intuitively, it would have been much nicer if we had more flexibility in choosing these Gradient Filters. Since, on an image where the edges are weak one would like a higher order Gradient than DOG in order to get high response at the edges which are not too priminant.However a LOG might be too susciptible to noise, but due to unavailability of other options one has to rely on poorly depicted result obtained using LOG. \\

The FDOG filters are designed using concepts from fractional order calculus. Similar filters have been designed in the frequency domain and has been practiced frequently in various control applications. Acharya et.al.~\cite{Acharya:2014:ECA:2537167.2537260} proposed a structured exact implementation of arbitrarily chosen cut-off based filters. We extend this idea to design a 2-D convolution mask based on the general discrete approximation of the n-th order differentiation operator, represented by (~\ref{eq:eq1}).
%\\ The idea of [24] can be extended to 2-D applying the finite difference method in both the x and y direction as given by equation~\ref{eq1} %The proposed algorithm in [1] though gives a very precise implementation of Fractional Filters in Frequency Domain, though a direct implementation of that algorithmm may not be a good choise for the present problem set up since it is too much of work and computation in this context. Thus, this work is a direct extension of the idea proposed in [1] to design a small spatial convolution mask to approximate the Frequency counterpart reasnably and can achieve much of the desired goal. \\


\begin{figure*}[ht]
\centering
\includegraphics[width=4.1cm,height=4.6cm]{images/tns1.png}
\includegraphics[width=4.1cm,height=4.6cm]{images/tns2.png}
\includegraphics[width=4.1cm,height=4.6cm]{images/DOG_noisy.png}
\includegraphics[width=4.1cm,height=4.6cm]{images/FDOG_noisy.png}

\caption{\label{fig:quickcomp2}Edge detection using FDOG on a noisy image. From left to right: original image, smoothed with $\sigma=2$ Gaussian kernel, DOG edge detection and FDOG edge detection. It can be observed that FDOG outperforms DOG even on a noisy image.}
\end{figure*}

\begin{multline}
\label{eq:eq1}
\frac{\partial^vs(x,y)}{\partial x^v}=s(x,y)-vs(x-1,y) + 
\frac{v(v-1)}{2}s(x-2,y) \\-\frac{v(v-1)(v-2)}{6}s(x-3,y)+... ,\\
\frac{\partial^vs(x,y)}{\partial y^v}=s(x,y)-vs(x,y-1) + 
\frac{v(v-1)}{2}s(x,y-2) \\-\frac{v(v-1)(v-2)}{6}s(x,y-3)+...
\end{multline}

The gradient to be computed is thus given by the sum of the partial derivatives (Equation~\ref{eq:eq2}).
\begin{equation}
\label{eq:eq2}
\bigtriangledown^v=\frac{\partial^vs(x,y)}{\partial x^v}+\frac{\partial^vs(x,y)}{\partial y^v}=\bigtriangledown^v_x+\bigtriangledown^v_y
\end{equation}
where instead of restricting the order to be integer i.e. in case of DOG, $v=1$ and LOG $v=2$; we propose to let $v$ take any fractional value. Theoretically, $v$ should be limited to one decimal place to avoid mathematical intractability. Also, for efficiency, we restrict the number of terms in equation~\ref{eq:eq1} to three. Figure~\ref{fig:quickcomp} shows the result of applying FDOG of order $0.5$ for edge detection on a standard image taken from the Berkeley Segmentation Dataset. Figure~\ref{fig:quickcomp} also shows a DOG kernel based edge detection and a benchmark obtained by averaging over the five hand edge-detected versions of the same image. All the results are subjected to non maximal suppression and displayed in normalized scale for comparison purposes. As can be observed, FDOG of order $0.5$ seems to perform better than standard DOG operator visually. In other words, FDOG weeds out noise and reveals structural image information more clearly. Even in highly noisy images, FDOG seems to perform better, as is verified on an image (taken from the CSIQ image database \cite{larson2010most}) corrupted with white noise (Figure~\ref{fig:quickcomp2}).

%Though from a theoritical perspective one should only restrict upto one decimal place since the moredecimal places we consider the more number of Riemann Sheets are considered and it often becomes intractable to obtain an exact solution with too many Riemann Sheet to share a single pole and also 

%The more terms one consider the more accurate the results are going to be. However, since the primary goal was to find a more efficient strategy without increasing the computational complexity we propose to truncate the series after three terms. The mask thus obtained will esstentially be similar in size to the standard Gradient Mask used in case of LOG or DOG. 


%These kind of spatial approximations combined with some $\gamma$-correction has been efficiently used for the purpose of Image denoising and has proved to be sucessfull under the presence of extremely high noise which often is the case of various Astronomical Images[25].\\
%However, there has been no previous attempts to use the power of fractional derivative in spite of having this elegant and straightforward integer order approximation, for the purpose ofimage segmentation. The reason is most likely the unavailability of sraightforward implimentations under the lights of a segmentation dataset and which can be readily done as a pre-processing step of the segmentation task without any additional computational complexity.

%Before going into a detailed analysis, we show a preview of how FDOG performs in comparison to DOG, when applied to a standard image taken from the Berkeley Segmentation Dataset.

%Before introducing a formal algorithm and analytical performance evaluation let us first go through some visualization of the Fractional Derivative of Gaussian Operator (FDOG) on some standard images and compare the performance with the edge detector performance using the standard Derivative of Gaussian Operator (DOG). \\
%first, A standard image from the Berkley segmentation Dataset is considered. The goal is to match the benchmark image obtained by handsegmentation. All the fuctions has ben writen using Matlab R2013b version.  The Image Gradient has been computed using a FDOG operator of order 0.5 and using the standard DOG operator available in Matlab. 
%Figure~\ref{fig:smooth} shows the original image in Grayscale and the smoothed version of the image using a Gaussian Kernel with $\sigma$=1 i.e. 1 pixel wide. Fig.2 shows the result obtained after the application of the standard DOG operator and one obtained after applying the proposed FDOG of order 0.5. The benchmark is also provided for comparison. The segmentation benchmark for the image is obtained by averaging over the 5 handsegmented image of the same image. Both results are subjected to non maximal suppression and displayed in normalized scale for comparison purposes.











\subsection{Evaluating FDOG Edge detection}
The standard measure to evaluate the performance of an edge detector is to measure the Peak Signal-to-noise Ratio (PSNR)~\cite{Canny:1986:CAE:11274.11275}. This is an effective measure when the noise models of an image are provided, or more generally if the imaging circumstances are known before hand and the detected edges can be clearly classified as true edges or noise. A more practical and widely adopted approach for any arbitrary given image is to filter the image and measure the structural loss caused therby. It assumes a general framework of the corrupted image as given in equation~\ref{eq:snr2}. %We use a performance measure effective in general cases and especially when we are concentrating on the end result of image segmentation.

%The results can be obtained following the approach in [10] and letting the order of the filter to be a variable and should be straightforward. However, this approach of evaluation is proper while establishing the superiority of an edge detector under the assumption that the Noise model is known. While, this approach might be reasonable when the sole goal is to build the edge detector. However, the main agenda of this paper is to come up with a improved version of the edge detection operation under the set-up that the goal is to perform segmentation on a dataset. Given this assumption that one does not have the Noise Models for the images it is utmost important to come up with a measure that can be readily evaluated against a dataset. Keeping this objective in mind a evaluation scheme is proposed which takes into account all the desirable properties for a good edge detection scheme as mentioned in section 4.1, but based on the assumption that segmentation is to be done on a datset and the Noise Models for images are not available i.e. the images might be taken under different surrundings and may be using different image acquisition devices. 

%\subsubsection{Peak Signal to Noise Ratio(PSNR)}

% This measure has been quite widely used in different Signal and Systems theory research as well. However, in order to measure this one must start with a noise model and do these calculations accurately. However, one does not have access to the uncorrupted image and also it is impractical to do the SNR calculations over the entire dataset since the images might be taken from various sources under different conditions and using different acquisition devices. Thus, 

\begin{equation}
\label{eq:snr2}
x[n]=s[n]+w[n]
\end{equation}

where $x[n]$ is the given image and $s[n]$ is the filtered one. The PSNR is then defined as shown in Equation~\ref{eq:snr3}.
\begin{equation}
\label{eq:snr3}
\begin{split}
PSNR=10log_{10}\frac{max(s^2[n])}{MSE}, 
\\
MSE=\frac{1}{MN}\sum_{i=1}^{M}\sum_{j=1}^{N}[\hat{s}(i,j)-s(i,j)]^{2}
\end{split}
\end{equation}

where $s[n]$ is the maximum signal value, typically $255$ when considering image pixel values, $M$ and $N$ are the height and width of the image, $\hat{s}$ is the processed image and $s$ is the original image, and MSE is the mean squared error.
%However, one drawback of this measure in the present problem set-up is that it does not take into account any Spatial information, however, in the present set-up the aim is to find a good measure to measure the structural content retention rather than the .

%Another popular option is to measure the Mean of squared error(MSE) between the image before and after processing (Equation~\ref{eq:snr4}).

%
%where $\hat s$ is the filtered output and $s$ is the input image. A major problem of using MSE alone is its dependency on the actual image itensity values[29].

%Another measure that has been widely used in measuring the image or video quality in case of image compression is the Peak Signal to Noise Ration[27](PSNR) which is similar to SNR but with the slight modification (Equation~\ref{eq:snr5}) that it takes into account the maximum squared intensity of the signal, as compared to the average one in case of SNR thus making it less constrained and more reasonable measure of the structural information lost during the process.

%

%where SNR looks at the ratio of the strengths of signal and noise,a direct extension from the concept of electrical power;but the PSNR takes into consideration the signal peak thus it is much more appropriate to this context. The justification is that here the main consideration is that how well high intensity regions come throught the noise rather than how does the algorithm performs under low intensity.\\
%Many other versions of the PSNR has been widely used, [15[29] almost all of which require some pre-assumptions computationally complex. While these are effective in image or video quality assessment, but in the context of the problem of segmentation it is sufficient to contain ourselves to PSNR since the goal is to compare the performance of different gradient orders. 

%\subsubsection{Detection Error}
While PSNR gives us an idea of how much structural information is retained in the gradient operated image, another criterion of good detection is to minimize the effect of noise. This can be addressed using the idea of False Discovery rate (DE)~\cite{citeulike:1042553}, which is given in equation~\ref{eq:DE}.
%a ratio of misclassified points as edges to misclassified points as non-edges should be minized. Thus, the second evaluation metric taken in to account is the product of Type-I and Type-II error i.e. Probability of misdetection and False alarm.
\begin{equation}
\label{eq:DE}
DE=P_m*P_f 
\end{equation}
where $P_m$ and $P_f$ are respectively Probability of missed detections and probability of false positives. A low value of this product implies good detection i.e. better edge detector.   

\subsubsection{Finding the optimal Gradient order}
The correct order of the gradient to be used in FDOG is data specific and should be optimized over all the images in the dataset. Thus finding the optimal order of the derivative can be now viewed as an optimization task with th score function, $J=\frac{PSNR}{DE}$ to be maximized.
Any standard approach like gradient descent can be used to find the optimal order. We restrict the search space to within one decimal place i.e. $v$ can only take values in steps of $0.1$ and select the order with highest score.
%Since, firstly, the search space is restricted and secondly, the corresponding filter weights arer pre-computed or can be computed parallaly using the general taylor series expansion equation provided in section 4.1 and thirdly, these can be reproduced in the frequency domain with nice and strong anlytical closed form results as shown in [1]. Incurring random co-efficients results in non-realizable filters in extremely higher order Riemann Sheets. 
Applying our algorithm to various datasets like the berkley segmentation dataset~\cite{937655}, The Stanford backgrounds dataset~\cite{5459211} and CSIQ noisy database it is found that in most cases the optimal order turns out be in the range 0.5-0.8 with lower order for highly noisy images like astronomical images. %Also a higher value is desired if the images have a very poor contrast i.e. taken under very low illumination settings. thus, on any standard datset one can assume an order of 0.5-0.8 without much loss of generality. However, for obvious reasons it is preferable to find the optimal order using gradient Descent or some kind of optimization technique. A detailed practical example has been given tyo demonstrate various parts of the algorithm on the Stanford Backgrounds Dataset in section[6]. 
%\\As an exemplary case the Stanford Backgrounds dataset isd considered and the approximate optimal order is found to be 0.7.
\begin{figure}[h]
\centering
\includegraphics[scale=0.32]{images/filter_score.png}
\caption{\label{fig:optimalorder}Performance of different Gradient Orders on Stanford Backgrounds Dataset}
\end{figure}

Figure~\ref{fig:optimalorder} shows the plot of score function with respect to different filter orders applied on the Stanford background dataset. The score function for each order have been computed over all the images and averaged to produce the reported value. It can be seen that the approximate optimal order is somewhere around 0.5-0.8. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%-------------NEW-------------------%%%%%%

%In order to validate our scoring scheme we also provide an evaluation on the BSDS500 using the Precision Recall Curves as an evaluation metric.  


%%%%%%-----Precision Recall Definition----
%%%%% Copied From 
%%% BSDS 500 @InProceedings{MartinFTM01,
%  author = {D. Martin and C. Fowlkes and D. Tal and J. Malik},
 % title = {A Database of Human Segmented Natural Images and its
 %          Application to Evaluating Segmentation Algorithms and
  %         Measuring Ecological Statistics},
  %booktitle = {Proc. 8th Int'l Conf. Computer Vision},
  %year = {2001},
  %month = {July},
  %volume = {2},
  %pages = {416--423}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%-----COPIED-----------------------

In order to validate our scoring scheme, we also generate a precision-recall curve for detection (Figure~\ref{fig:precrec}, Table~\ref{table:table1}). First we threshold the generated boundary map into several levels and at each level compute the precision, which is the probability that a machine generated pixel is a boundary pixel, and recall, which is the probability that a true boundary pixel is detected~\cite{937655}. The precision-recall curve reflects the inherent trade-off between misses and false positives. It would be nice to be able to compare the curves for different algorithms in terms of a single number. In an attempt to do so we introduce the F-measure, which is the harmonic mean of precision and recall, as a yardstick for an algorithm's performance. In general, for two algorithms whose curves are roughly parallel, the one furthest from the origin dominates the other. The F-measure is defined at all points on the precision-recall curve.  We report the maximum F-measure value across an algorithm's precision-recall curve as its summary statistic.
These results should not be considered as edge detection results since these are based on just computing the raw local gradients with different orders using \ref{eq:eq1} and does not apply any processing before feeding to the benchmarking and thus the results would be lower than that in the BSDS leader-board. However, we use these PR curves as a way of comparing the descriptive power of different gradient orders to validate our formulated evaluation metric based on PSNR and FDR.

%Nevertheless, we do need to threshold the boundary map in order to compare it to the ground truth boundaries, but we do so at many levels, e.g. 30.  At each level, we compute two quantities -- precision and recall -- and in this manner produce a precision-recall curve for the algorithm.  Precision and recall are similar to but different from the axes of ROC curves.  Precision is the probability that a machine-generated boundary pixel is a true boundary pixel.  Recall is the probability that a true boundary pixel is detected.  We consider these axes to be sensible and intuitive.  Precision is a measure of how much noise is in the output of the detector.  Recall is a measure of how much of the ground truth is detected.   The curve shows the inherent trade-off between these two quantities -- the trade-off between misses and false positives -- as the detector threshold changes.
%Although the precision-recall curve for an algorithm is a rich descriptor of its performance, it is still desirable to distill the performance of an algorithm into a single number.  This is possible to do in a meaningful way for algorithms whose curves do not intersect and are roughly parallel.  When two precision-recall curves do not intersect, then the curve furthest from the origin dominates the other.  The summary statistic that we use is a measure of this distance.  It is the F-measure, which is the harmonic mean of precision and recall.  The F-measure is defined at all points on the precision-recall curve.  We report the maximum F-measure value across an algorithm's precision-recall curve as its summary statistic.
Figure~\ref{fig:precrec} shows the precision-recall curves for varying orders and the variation of F-number with varying filter orders.  Intuitively, and also as the curves show, an increased order enhances more noisy peaks and too small an order fails to mine structural information. From the training images it is observed that 0.6 gives the best F-score of 0.523 which is almost 1\% improve over DOG. Whereas the LOG performs way bad and gives an F-score of 0.480 - almost 4\% less than the best. We use the Filter order as 0.6 on the test images to generate the precision-recall curve and also provide the precision-recall of the standard DOG for comparison purposes in Figure~\ref{fig:precrec}.
%It is straightforward to think about the nature of the Gradient Operator looking at the Filter weights. As one would expect that on increasing the order of the Gradient Operator one would see more noisy peaks emerging and true edges being suppressed. However, too small an order might also lead to bad results since as we go towards zero, the Gradient Filter weights become smaller and smaller and approach towards constancy extracting no or minimal structural details. In contrary, Increasing the order means increasing the relative weights of the Gradient Operator and as a result it might be more prone to noise. Fig. 6 shows an example demonstrating this by varying the Filter Order from 0.1 to 0.9.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%------------COPIED------------------------------%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}
\centering
\includegraphics[scale=0.235]{images/train.png}
\includegraphics[scale=0.235]{images/test.png}
%\includegraphics[scale=0.3]{images/bsds500.png}
\caption{\label{fig:precrec}Top:left: Precision Recall curves on training BSDS500 for Varying Gradient Order right: comparing PR curves for FDOG order 0.6 and DOG}
\end{figure}





%We first compute the Precision-Recall scores and the F-measures for different gradient orders varying from 0.2 to 2 in steps of 0.2 and found an optimal order at around 0.6. The precision Recall and the F-measures are provided in table[1]


\begin{table}[h]
\centering
\begin{tabular}{ |c|c|c|c| } 
 \hline
Gradient Order &  ODS & OIS & AP \\ 
 \hline
0.2 & 0.501 & 0.535 & 0.288 \\ 
0.4 & 0.506 & 0.538 & 0.311 \\ 
0.6 &  0.523 & 0.555 & 0.311 \\ 
0.8 &   0.518 & 0.552 & 0.404 \\ 
1 &    0.514 & 0.549& 0.370 \\ 
1.2 &  0.510 & 0.544 & 0.338 \\ 
1.4 & 0.508 & 0.546 & 0.266 \\ 
1.6 & 0.497 & 0.530 & 0.419 \\ 
1.8 & 0.495 & 0.536 & 0.329 \\ 
2 & 0.480 & 0.513 & 0.232 \\ 
  
 \hline
\end{tabular}
\caption{\label{table:table1} Precision-recall and F-measures}
\end{table}

Figure~\ref{fig:heli} shows the results of applying our FDOG filter with varying orders for edge detection.

\begin{figure}[h]
\centering
\includegraphics[height=3cm,width=4.1cm]{images/146074.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_groundtruth.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_02.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_04.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_06.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_08.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_10.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_12.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_14.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_16.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_18.png}
\includegraphics[height=3cm,width=4.1cm]{images/146074_20.png}
\caption{\label{fig:heli}The Result of varying the Gradient Order. Top Row: Original image (left) and ground truth (right). Second row: FDOG with v=0.2 (left) and v=0.4 (right). Each row shows an increase in order in steps of 0.2 from left to right. Thus, the last row has FDOG wth v=1.8 (left) and v=2.0 (right). }
\end{figure}





%\begin{figure}[h]
%\centering
%\includegraphics[height=3cm,width=4.1cm]{images/orig.jpg}
%\includegraphics[height=3cm,width=4.1cm]{images/groundT.png}

%\includegraphics[height=3cm,width=4.1cm]{images/p1.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p2.png}
%\includegraphics[scale=0.2]{images/p3.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p4.png}
%\includegraphics[scale=0.2]{images/p5.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p6.png}
%\includegraphics[scale=0.2]{images/p7.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p8.png}
%\includegraphics[scale=0.2]{images/p9.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p10.png}
%\includegraphics[scale=0.2]{images/p11.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p12.png}
%\includegraphics[scale=0.2]{images/p13.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p14.png}
%\includegraphics[scale=0.2]{images/p15.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p16.png}
%\includegraphics[scale=0.2]{images/p17.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p18.png}
%\includegraphics[scale=0.2]{images/p19.png}
%\includegraphics[height=3cm,width=4.1cm]{images/p20.png}

%\caption{\label{fig:Taj}The Result of varying the Gradient Order. The images follow the same ordering as Figure~\ref{fig:heli}}
%\end{figure}




==> CVPR /introduction.tex <==
\section{Introduction}
\label{sec:introduction}

%MOTIVATION-
A huge variety of modern computer vision algorithms are built on the computation of local derivatives of image brightness which provide local discriminative cues to scene structure, e.g., texture based segmentation~\cite{Malik:2001:CTA:543015.543016}, HOG based~\cite{1467360}, and SIFT~\cite{Lowe:2004:DIF:993451.996342} frameworks. Typically an input image is convolved with an image filter bank consisting of gradient filters in different orientations and scales. The response of these filters are used to construct a feature space which embeds structural image information.
%, e.g. by assembling normalized local orientation histograms in a dense grid over the image and feeding this feature to classifier like SVM. 
This approach is found to be incredibly powerful for detecting key image features or recognizing objects over different scales, appearances and poses. The success of these algorithms prove the importance of gradient orientations as a robust feature for  recognition~\cite{Shi:2000:NCI:351581.351611,Malik:1999:TCR:850924.851546, Malik90preattentivetexture, Blake:1987:VR:30394}. 
To date the most widely used gradient based features are extracted using the First Order Derivative of a Gaussian (DOG) kernel taken in different orientation and scales or considering the zero crossing in the response to the Laplacian of Gaussian Operator (LOG). As the order of the gradient operator increases, the response to edges is also higher, but an increased order also gives an undesirably higher response to noise or isolated points. In order to avoid noise enhancement images are often smoothed prior to edge detection. However, smoothing can cause a loss of structural information in some cases. Thus, choosing the proper gradient order for a given image depends largely on the image, e.g. we might want a weaker edge response for a noisy image and a stonger one for a crisp image.
%Again, if one has a highly noisy image (astronomical data, historical images) one might want to get weaker response that does not respond strongly to Noise i.e. gradient operator which gives weaker or smoother transition response at the edges might be useful. However, unfortunately unavailability of such Gradient Operators restrict the segmentation algorithm to either use DOG or zero crossing from LOG.

%APPLICATION-
%From the general understanding of image processing it is known that if one has an image where the edges are weak then  the gradient response should be able to find edges and retain structural information but should not be fooled by isolated points or noise i.e. should have low miss-detection. In other words it is desirable to have a edge detection framework which has high Signal to Noise Ratio but low Type-I and Type-II error. 
%\\Intuitively, this can be achieved by computing coarser local derivative. This would ideally improve the results of any edge detection, image segmentation algorithms that compute and use the gradient operator as a feature in the pipeline. Another possible application is in case of robust feature and texture matching problems which use gradient based algorithms because gradients are less susceptible o lighting and camera conditions and thus reduces the matching error.


\begin{figure}[h]
\centering
\includegraphics[scale=0.37]{images/01.png}
\caption{\label{fig:results1}Image segmentation using FDOG edge detector. From left to right: original image, true label and estimated label.}
\end{figure}


\begin{figure*}[ht]
\centering
\includegraphics[width=3.2cm,height=4.4cm]{images/test_smoothed1.jpg}
\includegraphics[width=3.2cm,height=4.4cm]{images/test_smoothed2.jpg}
\includegraphics[width=3.2cm,height=4.5cm]{images/bench.png}
\includegraphics[width=3.2cm,height=4.5cm]{images/DOG.png}
\includegraphics[width=3.2cm,height=4.5cm]{images/FDOG.png}
\caption{\label{fig:quickcomp}Edge detection using FDOG: Left to right: sample image, smoothed image, manual edge detection, DOG edge detection and FDOG with v=0.5. It can be observed that FDOG performance is closer to manual detection than DOG. }
\end{figure*}


In order to address this problem we propose a framework for generating a family of gradient operators with fractional orders, and show that the fractional gradients work better than integral ones for edge detection and eventual image segmentation. In order to design the fractional gradient operators, we use concepts from Fractional Calculus, which has been widely and efficiently used in the fields of signal processing. The fractional orders introduce higher order hyper-damped and ultra-damped poles which lends much more flexibility and accuracy in modeling complicated system dynamics~\cite{Acharya:2014:ECA:2537167.2537260,XX}.


%generalized family of Gradient operator in the context of Image segmentation which takes into account concepts from Fractional Calculus which has proven to be successful in a wide array of applications related to signals and systems over the past few decades. It successfully explains many real world phenomenon and often proven to be better models of real world system dynamics due to its added capability of providing more accurate description as compared to the integer dynamical systems. The added power of Fractional Order systems is due to the additional poles in Higher Riemann Sheets which often contribute to the important characteristics of a System~\cite{Acharya:2014:ECA:2537167.2537260}. Hence considering the poles in Higher Order namely Hyperdamped and Ultra-Damped Poles give more flexibility and accuracy in modeling complicated system dynamics[2],[3],[4]. It has been shown in~\cite{Acharya:2014:ECA:2537167.2537260} that Fractional Filters can be realized in a systematic approach in the Frequency Domain. However, the use of Fractional Order Filtering concepts has largely been restricted to the fields of Control System and Applied Mathematics. There have been very few attempts to use the power of Fractional Domain concepts in the computer vision.
%\subsection{Main Contribution}
In essence, we use fractional order gradients for designing fractional order derivative of Gaussian (FDOG) filters and show that our design achieves better edge detection performance than existing integer order gradient filters (Figure~\ref{fig:quickcomp}). In order to validate this performance gain, we apply our method to image segmentation (on images from Stanford Backgrounds Dataset~\cite{Koller:2009:PGM:1795555}, an example shown in Figure~\ref{fig:results1}) by building Histogram of Gradient Orientation (HOG) features on top of the FDOG filters, and learning a Markov Random Field based Model using Tree Re-weighted Belief Propagation based on the approach proposed in~\cite{10.1109/TPAMI.2013.31}. 

The rest of the paper is organised as follows: Section~\ref{sec:imsegment} gives a detailed description of the design of FDOG filters and demonstartes its performance on test images. Section~\ref{sec:learning} describes how the FDOG based approach can be used for image segmentation and Section~\ref{sec:results} depicts the performance gain for the same over existing methods, followed by a conclusion in Section~\ref{sec:conclusion}.

==> CVPR /learning.tex <==
\section{Image Segmentation using FDOG}
\label{sec:learning}

%In the field of Computer Vision graphical Model based approaches have gained much popularity of late in Computer vision problem since it is intuitively natural to think an image as a graph structure where each pixel can be considered as the nodes of the Graphical Model.However like most of the interesting problems  exact inference is usually intractable or NP- hard problem due to the high tree-width of the graph structure. Learning the graph structure is also intractable in most cases.[40] Many previous research work has been focused on approximating the likelihood [41].
%\\ However, a much recent work by Domke et.al. [41] reveals that the Learning/ parameter fitting can be viewed as repeated inference problem using the marginalization based loss function, which directly relates to the quality of prediction of a given marginal inference algorithm[42][43] also it seems to work better intuitively because it takes into account the approximation error and also it is robust to model mis-specification[41]. 
%\subsection{Background}
%In the past decade image representation using %graphical models [40,41] and
%Markov Random Field(MRF) have been widely used in wide array of vision problems [44]. %Blake et.al. provides a nice demonstration of the power of MRF in solving vision problems in [44]. %Broadly MRF can be treated as a tool for modeling the image data and difference inference algorithms when coupled one can make inferences about the image.

Image Segmentation is one of the most important application areas in Computer vision. Most of the image segmentation algorithms often use gradient based cues as features. In this section we apply the proposed fractional gradient based approach to an image segmentation task and evaluate its performance against state-of-the-art.

It is a common and successful practice to use Conditional Random Field (CRF) based approach in solving the segmentation task -it is also intuitively natural to think an image as a graph structure where each pixel can be considered as the nodes of the Graphical Model.
CRFs are a probabilistic framework for labeling and segmenting structured data (equation~\ref{eq:CRF}), such as sequences, trees and lattices. 

\begin{equation}
\label{eq:CRF}
P(X\mid Y)=\frac{1}{Z(Y)}\prod_C\psi(X_c,Y)\prod_i\psi(X_i,Y)
\end{equation}

The underlying idea is that of defining a conditional probability distribution over label sequences given a particular observation sequence, rather than a joint distribution over both label and observation sequences. 

However like most of the interesting problems  exact inference is usually intractable or NP- hard problem due to the high tree-width of the graph structure. Learning the graph structure is also intractable in most cases~\cite{Koller:2009:PGM:1795555}. Many previous research work has been focused on approximating the likelihood. We particularly focus on the recent work of Domke et.al.~\cite{10.1109/TPAMI.2013.31} where the Learning/ parameter fitting is viewed as repeated inference problem using the marginalization based loss function, which directly relates to the quality of prediction of a given marginal inference algorithm~\cite{10.1109/TPAMI.2013.31} also it seems to work better intuitively because it takes into account the approximation error and also it is robust to model miss-specification.  

%The general idea is to represent an image as a collection of nodes where the nodes are individual or a group of pixels. Hidden variables are introduced to the model for explaining the pixel values. The statistical dependency between hidden variables is expressed by grouping the hidden variables explicitly where these groups often correspond to the edges of the graph. The Markov random Field(MRF) is then defined by a probability distribution defined over the graph structure defined in equation~\ref{eq:MRF} 
%\begin{equation}
%\label{eq:MRF}
%p(x)=\frac{1}{Z}\prod_C\psi(X_c)\prod_i\psi(X_i)
%\end{equation}
%where the first term corresponds to the factors over the set of cliques C of the Graphical structure whereas the other term refers to factors corresponding to individual random variable i.e. over the nodes of the graph.
%One can alwasys represent distributions like this as long as the Hammersely-Clifford theorem is satisfied[45] i.e. each configuration of x has non-zero probability and also that each random variables are indepedent of all other random variables given its immediate neighbours. however, 
%For the segmentation or labeling task he notion of conditional random field (CRF) is proven to be more appropriate[46]. %can be viewed as modeling the conditional distribution of the variables given the obsered variables. Thus the notion of conditional random field(CRF) comes. [46].


%Most of the problems in vision framework relates to infering over the graphical model where, one learns a 
After learning a CRF model $P(Y\mid X)$ the query is to find the most likely configuration $\hat{x}$ given the observations. One option is to use the idea of Bayes estimator using the notion of utility function ~\cite{nikolova2007model} which specifies the happiness of predicting $\hat{x}$ if $X^*$ was the true output.Then the problem reduces to an optimization task where one finds the $\hat{X}$ that maximizes the Utility function. 
\begin{equation}
\hat{X}=\arg \!\max_X\sum_{x^{*}}P(X^*\mid Y)U(X,X^*)
\end{equation}
It is also shown that using the utility function as the indicator function that is 1 when output equals $X^*$ and zero otherwise, then it reduces to MAP estimate ~\cite{nikolova2007model} i.e. if, $U(X,X^*)=I[X=X^*]$
\begin{equation}
\hat{x}=\arg\!\max_X P(X\mid Y) 
\end{equation}
However, in real examples it might require humongous amount of data for accurate prediction. Thus, in practice, a utility function that maximizes the Hamming distance i.e. the number of components in the output that are correct, is used. This framework is popularly known as Maximum Posterior Marginal(MPM)[48]. %If the conditional distribution is skewed at a certain configuration then MAP and MPM reduces to the same. 
%\subsection{Learning}
%The agenda of this work is to learn the parameters of the Graphical model using the observed data. to be specific, here the intent is not to learn the graph structure automatically which remains an ac tive research area but is not under consideration in this work.\\
In the context of the current problem of learning the graphical model parameters, we view Learning from an Empirical risk Minimization framework as proposed in \cite{10.1109/TPAMI.2013.31}. where as usual the Risk is given by equation~\ref{eq:risk}.

\begin{equation}
\label{eq:risk}
R( \theta )=\sum_{\hat{x}}L(\theta,\hat{x})
\end{equation}
where the Loss function $L(\theta,\hat{x})$ explains how good the fit is with parameter $\theta$.


%One classic loss function used widely is the Likelihood itself (equation~\ref{eq:lossfn}).
%Technically, loss should be minimized but one can use the terminology loss as likelihood and its approximations and hence to be maximized. 
%\subsubsection{Likelihood approximation}

%\begin{equation}
%\label{eq:lossfn}
%L(\theta,x) =log P(x;\theta)=\theta.f(x)-A(\theta)
%\end{equation}
%Here the gradient is given as
%\begin{equation}
%\frac{dL}{d\theta}=f(x)-\mu(\theta)
%\end{equation}


One can find exact marginals using tree structured graphs- which is not practical in case of graphs with high tree width such as the current problem in consideration because in that case finding the exact likelihood and its gradient becomes computationaly hard due to the log partition function and the marginals. One widely used approach to tackle this problem has been the use of markov chain Monte carlo to approximate the marginals or using Constructive Divergence based approaches\cite{carreira2005contrastive}\cite{stewart2008learning} which also suffers from large complexity
A more recent approach is to use approximate inference methods which can be viewed as approximating the partition function in the likelihood itself. Then it can be shown that the approximate marginals itself become the exact gradient of the Surrogate Loss. In recent literature Surrogate Loss seems to be widely used where the marginals being approximated by either Mean Field, Loopy Belief Propagation(LBP) or Tree-reweighted Belief Propagation (TRW).\cite{wainwright2006estimating}\cite{weinman2008efficiently}
If approximate log partition function is used that bounds the true log partition function then Surrogate Likelihood is proved to be bounding the true likelihood where Mean field based Surrogate Likelihood Upper bounds and TRW based Surrogate Likelihood lower bounds. Other than these there is Expectation maximization(EM) based approaches which is appropriate in case of incomplete data\cite{russell2006using}, saddle point based approximations\cite{tighe2010superparsing}, pseudo-likelihood based approaches\cite{kim2007robust} and Piecewise Likelihood\cite{koppula2011semantic}  etc. Another issue to be taken into consideration is model mis-specification which often might be unavoidable due to the complex nature of problems or deliberately in case when the true model has many parameters to fit the data which leads to many degrees of freedom thus reduction becomes necessary.

%Given a correct model, it assymptotically converges to true parameters, %Using tree structured graph, 
%where exact marginals can be found using tree structured graphs..However, this is not practical in case of graphs with high tree width such as the current problem in consideration because in that case finding the exact likelihood and its gradient becomes computationaly hard due to the log partition function and the marginals. One widely used approach to tackle this problem has been the use of markov chain Monte carlo to approximate the marginals or using Constructive Divergence based approaches[50][51] which also sufferes from large complexity.
%However, these are pretty expensive computationally. \\
%Recently the idea that caught widespread attention is the idea to compute the marginals using approximate inference method. 


%\subsubsection{Marginal Based Loss Function}
%As discussed before, though 
%Though likelihood based learning, given a well specified model will converge to the true parameters asymptotically, it is computationally intractable and thus the various approximate algorithms discussed in section 5.3.1 deals with this. However, another issue to be taken into consideration is model mis-specification which often might be unavoidable due to the complex nature of problems or deliberately in case when the true model has many parameters to fit the data which leads to many degrees of freedom thus reduction becomes necessary.
% In this circumstances marginal based loss function is found to be a better option.In an approximate model no 'true' parameters exists rather the idea is to consider how the model will be used. One might compute the approximate marginals using the approximate inference algorithms at test time and tries to maximize these predictions thus essentially fits to the paradigm of Empirical Risk Minimization. Some widely popular marginal losses are -\\

For this particular problem we chose to train the model using a Clique Loss as in the present setting it is intuitively more straightforward to think about clique based loss rather than univariate loss as proved by Wainwright and Jordan et.al.\cite{wainwright2008graphical} that due to the standard moment matching criterion of exponential families if the clique marginals are correct the joint distribution has to be correct though the joint distribution might be far off perfect even if the univariate marginals are perfect.It is defined mathematically as-
\begin{equation}
L(\theta,x)=-\sum_Clog\mu(x_c;\theta)
\end{equation}
which can be viewed minimizing the empirical risk of the mean KL-divergence of the true clique marginals to
the predicted ones.
%The intuition is same as the Univariate case, the difference is that here the Clique Loss measures the mean KL-divergence of the approximate clique marginal and the true clique marginal.

%{\bf Univariate Logistic Loss}-
%The Loss is defined w.r.t approximate marginals obtained using Approximate algorithms and theintuition is that this measures the average accuracy of all the univariate approximate marginals. 
%Mathematically the Loss is defined as -
%\begin{equation}
%L(\theta,X)=-\sum_ilog\mu (x_i;\theta)
%\end{equation}
%This can be viewed as Empirical Risk Minimization of the KL-divergence between the true and the approximated marginals since,

%\begin{multline}
%\sum_iKL(q_i\mid \mid\mu_i)=\sum_i\sum_{x_i}q(x_i)log\frac{q(x_i)}{\mu(x_i;\theta)}\\
%=Const.- E_q\sum_ilog\!\mu(x_i;\theta)
%\end{multline}

%{\bf Clique Loss}- In the present problem setting i.e. 
%image segmentation it is intuitively more straightforward to think about clique based loss rather than univariate losse and thus and it turned out to be the case as reported in [42] that Clique based approach led to the best results under a CRF framework for Image Labeling problem. The definition is similar to the univariate case and just a straightforward extension to the univariate surrogate loss defined mathematically as-
%\begin{equation}
%L(\theta,x)=-\sum_Clog\mu(x_c;\theta)
%\end{equation}

%The intuition is same as the Univariate case, the difference is that here the Clique Loss measures the mean KL-divergence of the approximate clique marginal and the true clique marginal. It has been shown by Wainwright and Jordan et.al. [59] that due to the standard moment matching criterion of exponential families if the clique marginals are correct the joint distribution has to be correct though the joint distribution might be far off perfect even if the univariate marginals are perfect. Marginal Based loss function is can accomodate the Hidden Variables by taking sum in the loss over the observed variables only. 

%\subsubsection{Truncated Fitting}
The next step is to do the inference which turns out to be tricky for graphs with high tree width which requires two operations- firstly the evaluation of the loss function, which is pretty straight forward and can be done simply by plugging the marginal obtained by running the inference algorithm into the loss function and secondly, one requires to know the gradient $\frac{dL}{d\theta}$. The gradient can be computed by solving a set of sparse linear equation which assumes that the optimization problem is exactly solved ,though in practice one has to set a threshold to truncate which can be done very elegantly with a much lower computational expense by forming the learning
objective in terms of the approximate marginals obtained
after a fixed number of iterations. ~\cite{10.1109/TPAMI.2013.31}  

%we use the popular truncated fitting strategy on training set.

%For graphs with high tree width training requires firstly evaluation of the loss function, which is pretty straight forward and can be done simply by plugging the marginal obtained by running the inference algorithm into the loss function. Secondly, one requires to know the gradient $\frac{dL}{d\theta}$. It has been shown by Domke et.al. [42] that this can be obtained easily by solving a set of sparse linear equation. The proposed theorem in [41] reduces to the following.\\

%{\bf Theorem 1}\\
%Suppose, 
%\begin{equation}
%\mu(\theta):=\arg \! \max_{\mu:B\mu=d}\theta.\mu+H(\mu)
%\end{equation}
%Defining, 
%\begin{equation}
%L(\theta,x)=Q(\mu(\theta),x)
%\end{equation}
%and 
%\begin{equation}
%D=\frac{d^2H}{d\mu d\mu^T}
%\end{equation}
%It can be shown that,
%\begin{equation}
%\frac{dL}{d\theta}=(D^{-1}B^T(BD^{-1}B^T)BD^{-1}-D^{-1})\frac{dQ}{d\mu}
%\end{equation}
%owever, it was also shown in [42] that one does not need to form the constant matrix B explicitly or need not solve the system of equation explicitly as well. It can be shown using the standard Jacobian formation using finite differences that the Loss Gradient can be found as a simple limit given by,
%\begin{equation}
%\frac{dL}{d\theta}=\lim_{r\rightarrow 0}\frac{1}{r}(\mu(\theta+r\frac{dQ}{d\mu})-\mu(\theta))
%\end{equation}


%However, this assumes that the optimization problem is exactly solved However, in practice one has to set a threshold to truncate. It can be done elegantly with a much lower computational expense forming the learning
%objective in terms of the approximate marginals obtained
%after a fixed number of iterations.

It leads to a series of simple structured steps viz. Inputting parameters, applying the iterations of either
TRW or mean field, computing predicted marginals,
and finally the loss are all differentiable operations.
Here we use back-propagating Tree Re-weighted Belief Propagation Framework which calculates the marginals and plug them into the marginal based loss after a certain number of iterations even if the inference algorithm did not converge, which is possible because each step is differentiable.  
%Thus,
%the loss gradient is efficiently computable, at least in
%principle, by reverse-mode automatic differentiation proposed by Stovanov et al. [60] However, one major drawback of autodiff is it's large memory requirement which can be efficiently reduced using the Backnorm Operator defined by
%\begin{equation}
%backnorm(a,b)=b\odot (a-a.b)
%\end{equation}
%Using the backnorm operator Backpropagating inference algorithms such as Back Mean Field and Back TRW can be derived. 
%The basic intuition here is that even if after a certain number of iterations the inference algorithm does not converge one calculates the marginals and plug them into the marginal based loss. This is possible because each step in this process is differentiable, this specifies
%the loss as a differentiable function of model parameters.

After execution of Back TRW %it can be shown that
the parameter $\theta(x_c)$ for the clique based loss can be represented mathematically as  
%\begin{equation}
%\overleftarrow{\theta}(x_i)=\frac{dL}{d\theta(x_i)}
%\end{equation}
%and
\begin{equation}
\overleftarrow{\theta}(x_c)=\frac{dL}{d\theta(x_c)}
\end{equation}



==> CVPR /results.tex <==


\subsection{Experimental Results of using FDOG for segmentation}
\label{sec:results}




%In order to experiment with our proposed FDOG based method we chose a difficult dataset where there is a lot of scope for improvement from the state of the art. We briefly explain each step of the experiment in subsequent sub-sections.
In order to experiment with our proposed FDOG based method we have chosen the Stanford background dataset which has 715 images of outdoor scenes taken from different publicly available datasets like LabelMe, MSRC, PASCAL VOC and Geometric Context; each image of resolution approximately 240 * 320. Most pixels are labeled one of the eight classes with some unlabeled. 
%\subsection{Feature Selection}
%he main agenda of this work was to establish FDOG based approach as an unified approach tto improve any edge detection based segmentation algorithm. For that reason in order to demonstrate that and a fair comparison solely based on the way the gradient features being calculated. Thus, we stick to features similar to the work that currently leads on this Dataset[42]. 
All the experiments have been done on a Dual Core, 3GHz Processor with parallel tasks running on both the processor.
We have sticked with the simple features used in the state-of-the-art algorithm \cite{10.1109/TPAMI.2013.31} with replacing the gradient computations by our method in order to demonstrate the success of the proposed algorithm. 
The experimental method has the following flow chart.
\begin{enumerate}
\item We have used a pairwise 4 connected grid model.
\item We found the appropriate order of the Gradient Operator to be 0.7 using the score Function described in Section~\ref{sec:imsegment}. To run over all images and compute the approximate one decimal approximate of FDOG it took about 5 minutes.
\item For the unary features we first computed RGB intensities of each pixel, along with the normalized 
vertical and horizontal positions. We expand these initial features into a larger set using sinusoidal expansion, specifically use sin(c.s) and cos(c.s) where s is the initial feature mentioned for all binary vectors c of appropriate lengths leading to total 64 features. \cite{konidaris2011value}
\item Compute FHOG (fractional HOG)i.e. Histogram of Oriented gradient Features but the gradients are found using the proposed method i.e. using a third order approximate kernel using ~\ref{eq:eq1} where the order was taken as 0.6.
\item For Edge Features between pixels i and j we considered 21 base features comprsinga constant of one,Euclidian Norm of RGB value difference dicretized into 10 levels and maximum response of FDOG at i or j over three channels and aging binning into 10 dicrete levels and one feature based on the difference of RGB intensities.
\item All methods are trained using TRW to fit the Clique Logistic Loss. 
\end{enumerate}

Apart from using FDOG we also change the Optimization algorithm to R-PROP for improved computational efficiency.






\subsection{Performance}
The model is trained with 90 Images in a Monte Carlo Manner with 10 fold cross validation splitting the Training Set into Training and Validation in 90:10 ratio and the data was also shuffled randomly to avoid pathological ordering. The training took around 5 hours on a Intel dual core 3GHz Processor. The training performance is shown in Figure~\ref{fig:tperf}

\begin{figure}
\centering
\includegraphics[scale=0.2]{images/final_results_train_error.png}
\caption{\label{fig:tperf}Training Performance of the Model.}
\end{figure}
The TRW BP approach by Domke et.al ~\cite{10.1109/TPAMI.2013.31} using same set of features but HOG and and edge detectors use DOG is the state of the art 22.1\% average error on test data. We bettered that in our experiments reducing the error by almost 10\%. Our average error on the test data turned out to be 20.8\%. Table~\ref{table:table2} shows the result on Stanford Dataset. Some visual results on test data are shown in Figure~\ref{fig:results}
%However, though it improved the state of the art by reducing the error by about 10\% , this can be streched a further 5\% if could be learnt on more training images\\
\begin{figure}
\centering
\includegraphics[scale=0.45]{images/8.png}
\includegraphics[scale=0.45]{images/7.png}
\includegraphics[scale=0.45]{images/5.png}
\includegraphics[scale=0.45]{images/02.png}
\includegraphics[scale=0.45]{images/03.png}
\includegraphics[scale=0.45]{images/4.png}
\includegraphics[scale=0.45]{images/6.png}
%\includegraphics[scale=0.45]{images/9.png}
\includegraphics[scale=0.364]{images/11.png}
\includegraphics[scale=0.364]{images/12.png}
\includegraphics[scale=0.364]{images/13.png}
\caption{\label{fig:results}Image segmentation. Each row, from left to right: original image, true label and estimated label.}
\end{figure}


\begin{table}

  \caption{Comparison with different algorithms}
  \centering
\begin{tabular}{|l|c|r|}
\hline
Algorithm & Avg. Accuracy\\\hline
Region-based energy\cite{konidaris2011value} & 65.5 \\\hline
Stacked Labeling \cite{gould2009decomposing} & 66.2\\\hline
RGB-D \cite{munoz2010stacked} & 74.5\\\hline
TRW BP+Clique Loss \cite{10.1109/TPAMI.2013.31} & 77.9\\\hline 
TRW BP+ CLique Loss+ FDOG [us]& 79.2\\\hline \hline
\end{tabular}
\label{table:table2}
\end{table}



\section{Discussion and Future Work}
\label{sec:conclusion}
As can be seen from the demonstrated results we have done quite well on the difficult Stanford Backgrounds Dataset. Though 20.8\% error is quite high, there is a lot of room for improvement. The reason for this improvement is the efficient calculation of Gradient Features and it can improve the performance of any of the existing algorithms that are based on Gradient Features. Some of the future work in this might be to extend the concept directly from Frequency Domain and see how it affects the performance. Some, other datasets can be explored. Also, one important option is to apply the Texture Based Approach using this framework as intuitively it seems to be a more realistic idea in case of Contour Based Edge Detection. We believe that using this unified framework the Texton Based approach can also be improved by a few notch.   


==> FOC.tex <==
\section{Fractional Order Calculus Overview}
\label{sec:FOC}

It is actually a more simplified framework rather a subset of the complex Calculus which says that Diff-integral operators can take any complex value. thus, the integer order diff-Integral operators belong to the integer domain which lies inside a single Riemann Sheet  of Fractional domain which in turn falls within the superset of complex calculus.\\
In spite of the fact that fractional order calculus was introduced 300 years ago but still most of the notions remain unclear and unrealizable. For example, if one considers a filter of orer 1 it implies 1 pole in the integer oreder Frequency domain, but it might be mapped as $\frac{10}{10}$ i.e. 10 poles distributed over 10 riemann sheets , both seem to give similar response thus are equivalent. Thus, on a higher level it can be said

\begin{equation}
\{Integer Domain\} \subseteq \{Fractional Domain\} \subseteq \{Complex Domain\}
\end{equation}


"Fractional Calculus is a field of applied mathematics that deals with
derivatives and integrals of arbitrary
orders (including complex orders), and
their applications in science, engineering, mathematics, economics, and
other fields" [4]
The idea of Fractional Calculus dates back to 17th Century. The term was first coined by L'Hospital to Leibnitz while discussing about the possible interpretation of his derivation of $n^{th}$ order derivative.[2] And the first breakthrough was provided by Liebnitz when he introduced a possible approach to Fractional Order Differentiation(1697) \\
\begin{equation}\frac{d^n e^{mx}}{dx^n}=m^ne^{mx} \end{equation}
\\
Later Euler(1730)  suggested using the relationship for negative or non integer(rational) values for m=1 and n=1/2;
\\
\begin{equation}\frac{d^n x^m}{dx^n}=\frac{\Gamma (m+1)}{\Gamma (m-n+1)}x^{m-n}\\ \frac{d^{1/2}x}{dx^{1/2}}=\frac{2x^{1/2}}{\sqrt{\pi}} \end{equation}\\
While Euler proved it for specific value n=1/2 it was still not sure whether it exist for all the fractional orders and if there is something that can be applied generally and the first step in generalizing the concept for any non-integer order was given by Fourier (1820-1822) when he proposed the general n th order differentiation is given as\\
\begin{equation}\frac{d^nf(x)}{dx^n}=\frac{1}{2\pi}\int_{-\infty}^{\infty}f(z)dz\int_{-\infty}^{\infty}p^ncos(px-pz+n\frac{\pi}{2})dp \end{equation} 
\\
Since then many top Mathematicians (Pure and Applied) of their times have contributed significantly in this field namely N. H. Abel, M. Caputo, L. Euler, J. Fourier, A. K. Grunwald J. Hadamard, G. H. Hardy, O. Heaviside, H. J. Holmgren,
P. S. Laplace, G. W. Leibniz, A. V. Letnikov, J. Liouville, B. Riemann
M. Riesz, and H. Weyl etc.[4]. 

\subsection{Popular Fractional Differ-Integrals}
The main results on fractional Diff-Integrals that are widely used and popular are provided briefly.[1][2]
\subsubsection{Grunwald–Letnikov (G–L) definition}
This is basically an extension of the backward finite
difference formula for successive differentiation. This
formula is used widely for the numerical solution of
fractional differentiation or integration of a function.
According to Grunwald–Letnikov definition the $\alpha^{th}$ order differ-integration of a function f(t) is defined as 
\begin{equation}
D_t^{\alpha}f(t)=lim_{h\rightarrow 0}\frac{1}{h^{\alpha}}\sum_{j=0}^{\infty}(-1)^j \frac{\Gamma(\alpha +1)}{\Gamma(j+1)\Gamma(\alpha-j+1)}f(t-jh)
\end{equation}
\subsubsection{ Riemann–Liouville (R–L) definition}
This is an extension of n-fold successive integration. The $\alpha$-th order differentiation of f(t) is defined as 
\begin{equation}
D_t^{\alpha}f(t)=\frac{1}{\Gamma(n-\alpha)}\frac{d^n}{dt^n}\int_{\alpha}^{t}\frac{f(\tau)}{(t-\tau)^{\alpha -n +1}}d\tau   
\end{equation}

